Computing Optimal Coarse Correlated Equilibria in Sequential Games

We investigate the computation of equilibria in extensive-form games where ex ante correlation is possible, focusing on correlated equilibria requiring the least amount of communication between the players and the mediator. Motivated by the hardness results on the computation of normal-form correlated equilibria, we introduce the notion of normal-form coarse correlated equilibrium, extending the definition of coarse correlated equilibrium to sequential games. We show that, in two-player games without chance moves, an optimal (e.g., social welfare maximizing) normal-form coarse correlated equilibrium can be computed in polynomial time, and that in general multi-player games (including two-player games with Chance), the problem is NP-hard. For the former case, we provide a polynomial-time algorithm based on the ellipsoid method and also propose a more practical one, which can be efficiently applied to problems of considerable size. Then, we discuss how our algorithm can be extended to games with Chance and games with more than two players.

==> contents/exp.tex <==
\begin{table*}[t]
	\centering
	\small
	\caption{Comparison of the performance with the two different oracles.}
	\begin{tabular}{c||r|r|r|r|r|r|r|r|r|r|r|r}
		%\hline
		& \multicolumn{4}{c}{Game size} & \multicolumn{4}{|c|}{\textsf{P-LRC}} & \multicolumn{3}{|c}{\textsf{MI-LRC}}\\
		\hline
		Game & $|Q_1|$ & $|Q_2|$ & $|H_1|$ & $|H_2|$ & Phase1 & Phase2 & Time & Solved  & Phase1 & Phase2 & Time & Solved\\
		     &        &        &         &          & (steps) & (steps) & (sec)& (in 12h)& (steps) & (steps) & (sec) & (in 12h)\\
		\hline
		R5-3 & 126 & 102 & 43 & 35  & 5.6 & 8.9 & 8.10 & 20 & 5.8 & 3.1 & 0.3 & 20 \\
		R10-2 & 664 & 680 & 333 & 340 & 5.6 & 11.3 & 1125.0 & 20 & 5.9 & 6.4 & 23.4 & 20\\
		R12-2 & 2649 & 2697 & 1325 & 1349 & 5 & 7 & 39981.0 & 1 & 6.1 & 6.9 & 464.0 & 20\\		
		
		%\hline
	\end{tabular}
	\label{tab:confronto}
\end{table*}


\begin{table}[t]
  \setlength{\tabcolsep}{4pt}
	\centering
	\small
	\caption{Performance of \textsf{MI-LRC} on large two-player games and games with nature.}
	\begin{tabular}{c||r|r|r|r|r|r|r}
		%\hline
		Game & $|Q_1|$&$|Q_2|$ & $|H_1|$&$|H_2|$ & Phase1 & Phase2 & Time\\
		\hline
		R13-2 &  5364 & 5316 & 2682 &2659 & 6 & 5 & 1159.6\\
		\hline
		G3R & 58 & 58	& 47& 47 & 8 & 1 & 0.1\\
		G3S & 334 &334	& 274 &274 &  74 &  1 & 131.6\\
		G3D & 334 &334	& 274 &274 & 6 & 1 & 1.7
		%\hline
	\end{tabular}
	\label{tab:milp}
\end{table}


\section{Experimental Evaluation}\label{sec:exp}

We compare the performance of our column generation method with the two different oracles \textsf{P-LRC} and \textsf{MI-LRC} on random two-player general-sum games with utilities in $(-1,1)$.
%
Denoting by R$d$-$b$ games of depth $d$ and branching factor $b$, we generate 20 instances for each of the following configurations: R5-3, R10-2, R12-2, R13-2.
%
%We also test \textsf{MI-LRC} on instances of two-player games with Nature.
We also experiment on instances of two-player games with chance.
%
We employ \emph{Goofspiel} game instances~\cite{ross1971,saffidine2012}, a bidding game where each player has a hand of cards numbered from 1 to $K$. A third stack of $K$ cards is shuffled and used as prizes. Each turn a prize card is revealed, and each player chooses a private card to bid, with
the high card winning the current prize. After $K$ turns, all the prizes have been dealt out and the payoff of each player is the sum of the prize cards that they have won. In our experiments, we use $K=3$ (3 card ranks), with two different tie-breaking rules, namely, the players splitting the value of the card on the table equally (G3S) or discarding it (G3D).
%
G3R is the variant in which the order of the prize cards is known.

For the experiments, we employ the state-of-the-art MILP solver GUROBI (version 8.0).
%, using the AMPL modeling language (version 20180624).
%
The computations are run on a multi-processor system equipped with 16 dual 2.6 GHz Intel Sandybridge processors and 64 GBs of RAM.

We remark that the use of an LP defined directly on the normal form of a game (Definition~\ref{def:cce}) is impractical for every instance of our experimental setting due to its exponential size.
%
For instance, games like G3S and G3D contain more than $5\cdot 10^{13}$ variables.
%
For problems of this size, even building their LP formulation in memory is almost impossible (let alone solving it).
%
The column generation techniques we propose completely circumvent this issue.
%, as they only require to solve (sub)problems of polynomial size.

Table~\ref{tab:confronto} reports the average results that we obtained on the two-player instances of class R5-3, R10-2, and R12-2 with both \textsf{P-LRC} and \textsf{MI-LRC}.
%
The results obtained on the R13-2 instances, together with those for two-player games with chance, which are too large to be handled with \textsf{P-LRC}, are reported in Table~\ref{tab:milp}.

First, we notice that the number of columns generated before reaching optimality is always quite small.
%
This justifies even more the adoption of a column generation approach, since the algorithm requires only a few iterations to reach an optimal solution once a basic feasible solution is found.
%
Moreover, the results clearly illustrate that the \textsf{MI-LRC} oracle allows for a dramatic improvement in the performance of the algorithm.

Overall, our column generation method employing \textsf{MI-LRC} is able to compute a socially optimal NFCCE even on instances with more than 5000 cumulative sequences and 2500 information sets in less than one hour.
%
%In about 1000 seconds, we can solve random two-player games with over 5000 sequences and 2500 information sets.

%
%As we will argue in the concluding section, there may still be some margin for further improving the scalability of these techniques.


==> contents/inapproximability.tex <==
\section{Inapproximability of NFCE}\label{sec:5_inapprox}
\textsf{NFCE-SW} is kown to be \textsf{NP}-hard~\cite{vonStengel2008}. An open question is whether the problem can be approximated efficiently. We show that the answer is negative.
%Specifically, we further characterize the complexity of the problem by showing that the problem is unlikely to be approximable in polynomial time to within a factor polynomial in its size.

\begin{theorem}\label{th:sw_apx_hard}
	\textsf{NFCE-SW} is not in Poly-\textsf{APX} even in 2-players extensive-form games with perfect recall and without chance moves, unless $\textsf{P}=\textsf{NP}$.
\end{theorem}
\begin{proof}
Given a boolean formula in conjunctive normal form $\phi$ with $\eta$ clauses and $m$ variables, \textsf{MAX-SAT} is the problem of determining the maximum number of clauses that can be made true by a truth assignment to the variables of the formula. Denote by $\{c_1,\ldots,c_\eta\}$ the set of clauses belonging to $\phi$, and by $c^*$ the value of the optimal assignment for \textsf{MAX-SAT} over $\phi$. Clearly, $c^*\in\{1,\ldots,\eta\}$. Moreover, denote by $\{v_1,\ldots,v_m\}$ the set of variables appearing in $\phi$.
% costruzione
Let $\overline{c}\in\{1,\ldots,\eta\}$ be a given constant. We build an extensive-form game $\Gamma_{\overline{c}}$ with $N=\{1,2\}$ as follows, %(the structure of the tree is a non-trivial extension of the one adopted in~\cite{vonStengel2008}), 
where we denote by $x^i_j$, $a^i_j$, $h^i_j$, nodes, actions and information sets such that, respectively, $x^i_j\in V_j$, $a^i_j\in A_j$, $h^i_j\in H_j$:
\begin{itemize}[nolistsep,itemsep=0mm,leftmargin=.5cm]
	\item The root of the tree $x_2^0\in V_2$, is s.t., given $h_2^0\in H_2$, $x_2^0\in h_2^0$, $|h_2^0|=1$ holds. Moreover, $\rho(x_2^0)=\{a_2^{c_1},\ldots, a_2^{c_\eta}\}$, i.e., Player 2 has one action per clause at $x_2^0$.
	
	\item The second level of the tree is composed of $\{x_1^{c_1},\ldots,x_1^{c_\eta}\}$, where $\forall j\in\{1,\ldots,\eta\}$, $\chi(x_2^0,a_2^{c_j})=x_1^{c_j}$. On this level, there is a single $h_1^0\in H_1$ s.t., for all $x_1^{c_j}$, $x_1^{c_j}\in h_1^0$ and $|h_1^0|=\eta$.
	%
	% All $x_1^{c_j}$ belong to the same information set $h_1^0\in H_1$, which is s.t. $|h_1^0|=\eta$. 
	%
	Each $x_1^{c_j}$ has the following set of actions $\rho(x_1^{c_j})=\{a_1^{c_1},\ldots,a_1^{c_\eta},a_1^{T}\}$. 
	
	\item $\forall i,j\in\{1,\ldots,\eta\}$, $\chi(x_1^{c_i},a_1^{c_j})=l^{(i,j)}\in L$ (i.e., each action of Player 1 corresponding to a clause leads to a terminal node). $\forall l^{(i,j)}$, $U_1(l^{(i,j)}) = -1$ if $i=j$, and $U_1(l^{(i,j)}) = \frac{\eta\overline{c}+1}{\eta-1}$ otherwise, where $\overline{c}$ is the given constant. $\forall l^{(i,j)}$, $U_2(l^{(i,j)})=-U_1(l^{(i,j)})$.
	
%	\item $\forall i\in\{1,\ldots,\eta\}$, $\forall j\in\{1,\ldots,\eta\}$, $\chi(x_1^{c_i},a_1^{c_j})=l^{(i,j)}\in L$ (i.e., each action of player 1 corresponding to a clause leads to a terminal node). In terminal node $l^{(i,j)}$, $U_1$ is so defined: $U_1(l^{(i,j)}) = -1$ if $i=j$, and $U_1(l^{(i,j)}) = \frac{\eta\overline{c}+1}{\eta-1}$ otherwise,
%	\begin{scriptsize}
%	\begin{equation*}
%	U_1(l^{(i,j)}) = \begin{cases}
%	\begin{array}{ll}
%	-1 &\textnormal{if }i=j\\
%	\frac{\eta\overline{c}+1}{\eta-1} & \textnormal{otherwise}
%	\end{array}
%	\end{cases}
%	\end{equation*}
%	\end{scriptsize}
%	where $\overline{c}\in\{1,\ldots,\eta\}$ is a given constant. For each $l^{(i,j)}$, $U_2(l^{(i,j)})=-U_1(l^{(i,j)})$.
	
	\item $\forall i\in\{1,\ldots,\eta\}$, $\chi(x_1^{c_i},a_1^T)=x_2^i$. Each $x_2^i$ belongs to a singleton information set $h_2^i\in H_2$ and has an action for each literal $\pm v_j$ in $c_i$. We denote them by $a_2^{(i,+v_j)}$, $a_2^{(i,-v_j)}$, depending on how variable $v_j$ appears in $c_i$.
	
	\item $\forall i\in\{1,\ldots,\eta\}$, $\forall a_2^{(i,\pm v_j)}\in \rho(x_2^i)$ we have $\chi(x_2^i,a_2^{(i,\pm v_j)})=x_1^{(i,\pm v_j)}$. Each $x_1^{(i,\pm v_j)}$ belongs to $h_1^{v_j}\in H_1$. There is one information set $h_1^{v_j}$ for each of the $m$ variables. At $h_1^{v_j}$, Player 1 selects the truth assignment for $v_j$. $\forall x_1^{(i,\pm v_j)}$, $\rho(x_1^{(i,\pm v_j)})=\{T,F\}$, where choosing $T$ ($F$) means Player 1 sets $v_j$ to true (false). 
	
	\item $\forall i\in\{1,\ldots,\eta\}$, $\forall j\in\{1,\ldots,m\}$, $\forall k\in\{T,F\}$, $\chi(x_1^{(i,\pm v_j)},k)=l^{(i,\pm v_j,k)}\in L$. The utilities in these terminal nodes are defined as $U_2(l^{(i,+v_j,k)})=U_2(l^{(i,-v_j,k)})=0$ for each $k$, and:
	\end{itemize}

	\begin{small}
	\begin{equation*}
	U_1(l^{(i,+v_j,k)} = \begin{cases}
	\begin{array}{ll}
	\eta &\textnormal{if }k=T\\
	0 &\textnormal{if }k=F
	\end{array}
	\end{cases}, 
%	\end{equation*}
%	
%	\begin{equation*}
	U_1(l^{(i,-v_j,k)}) = \begin{cases}
	\begin{array}{ll}
	0 &\textnormal{if }k=T\\
	\eta &\textnormal{if }k=F
	\end{array}
	\end{cases}.
	\end{equation*}
	\end{small}


\noindent Notice that Player 1 has perfect recall since the information sets of type $h^{v_j}_1$ are only reached when she selects $a_1^T$.

% definizione strategia che da eq max-sat
Denote by $\Gamma'=(\{1,2\},P,U')$ the reduced normal-form of $\Gamma_{\overline{c}}$ (with $P=P_1\times P_2$). %, where $P_i$ is the set of reduced joint plans of player $i$ and, with a slight abuse of notation, $U_i:P_1\times P_2\rightarrow \mathcal{R}$. 
%
Let $\hat{\sigma}\in \Delta(P)$ be a probability distribution with the following properties:

\begin{property}\label{prop:pure}
	There exists $\overline{p}_1\in P_1$ s.t. $\sum_{p_2\in P_2}\hat{\sigma}(\overline{p}_1,p_2)=1$ and $\overline{p}_1\in \{a^T_1\}\times (\times_{j\in\{1,\ldots,m\}} \rho(h_1^{v_j}))$.%, meaning that a single truth assignment for variables in $\phi$ is selected.
\end{property}
\begin{property}\label{prop:uniform}
	For each $i\in \{1,\ldots,\eta\}$, there exists $\overline{p}_2^i\in \{a_2^{c_i}\}\times(\times_{j\in\{1,\ldots,\eta\}} \rho(h_2^j))$ s.t. $\sum_{p_1\in P_1} \hat{\sigma}(p_1,\overline{p}_2^i)=\frac{1}{\eta}$ (i.e., each $c_i$ is selected at the root with equal probability by Player 2 and a single literal for each clause $c_i$ is chosen).
\end{property}
\begin{property}\label{prop:max}	
	$\hat{\sigma}$ is the probability distribution maximizing the social welfare while satisfying Properties~\ref{prop:pure} and \ref{prop:uniform}.
\end{property}

Notice that $\hat{\sigma}$ provides a social welfare equal to $\eta\frac{c^*}{\eta}=c^*$. Let $\sigma^*$ be a solution to \textsf{NFCE-SW} over $\Gamma_{\overline{c}}$ (i.e., an NFCE maximizing the social welfare). During the construction of $\Gamma_{\overline{c}}$, we only required  $\overline{c} \in \{1,\ldots,\eta\}$. %In order to check whether $\hat{\sigma}$ is an NFCE for $\Gamma_{\bar c}$, we have to distinguish three cases w.r.t. the optimal value of \textsf{MAX-SAT} over $\phi$.
Now, we distinguish the following three cases w.r.t. the optimal value of \textsf{MAX-SAT} over $\phi$. In each of them, we provide some guarantees over the value provided by $\sigma^*$. In a second step, we will use this information to prove our result.


($\overline{c}<c^*$). In this setting, $\hat{\sigma}$ is an NFCE of $\Gamma_{\overline{c}}$. First, let us focus on Player 1. It is enough to compare $\overline{p}_1$ with another action $p'_1\in \{a^T_1\}\times (\times_{j\in\{1,\ldots,m\}} \rho(h_1^{v_j}))$, $p'_1\neq\overline{p}_1$, and an action $p''_1\in \{a_1^{c_1},\ldots,a_1^{c_\eta}\}\times (\times_{j\in\{1,\ldots,m\}} \rho(h_1^{v_j}))$. In the first case, NFCE constraints are not violated due to Property~\ref{prop:max}. In the second case, given $\hat{\sigma}$, Player 1 obtains, when choosing $p''_1$ in place of $\overline{p}_1$, utility $-\frac{1}{\eta}+\frac{\eta-1}{\eta}\frac{\eta\overline{c}+1}{\eta-1}=\overline{c}$. By playing $\overline{p}_1$, she obtains a return of $c^*$. Thus, since $\overline{c}<c^*$, Player 1 has no interest in replacing $\overline{p}_1$ with another normal-form plan. The same holds for Player 2 since $\hat{\sigma}$ assigns strictly positive probability only to outcomes of type $(\overline{p}_1,p_2)$, and $U_2(\overline{p}_1,p_2)=0$, $\forall p_2\in P_2$. Then, $\hat{\sigma}$ being an NFCE, $\sigma^*$ guarantees a social welfare $\geq c^*$.
	
($\overline{c}=c^*$). We claim that, in this setting, $\Gamma_{\overline{c}}$ admits only NFCEs that either have social welfare 0 or $c^*$. To show this, we first note that the only case in which a social welfare strictly greater than 0 is reached is when Player 1 selects $a_1^T$ at $h_1^0$. This requires Player 2 to play each action $a_2^{c_i}$ at $h_2^0$ with a cumulative probability of $1/\eta$ (i.e., Property~\ref{prop:uniform}). To see this, let $\sigma'\in \Delta(P)$ and assume that $a_2^{c_i}\in \rho(h_2^0)$ is played with probability \mbox{$\gamma=\sum_{p\in P_1\times (\{a_2^{c_i}\}\times_{j\in \{1,\ldots,\eta\}}\rho(h_2^j) )}\sigma'(p)< \frac{1}{\eta}$}. Then, by playing $a_1^{c_i}$ at $h_1^0$, Player 1 obtains $-\gamma + (1-\gamma)\frac{\eta\overline{c}+1}{\eta-1} > \overline{c}$, 
%	\begin{scriptsize}
%		\begin{align*}
%		& -\gamma + (1-\gamma)\frac{\eta\overline{c}+1}{\eta-1} > -\frac{1}{\eta} + \frac{\eta-1}{\eta}\frac{\eta\overline{c}+1}{\eta-1}=\overline{c}
%		\end{align*}
%	\end{scriptsize}
and, therefore, she would rather pick $a_1^{c_i}$ over $a_1^{T}$.
%
Now, since Property~\ref{prop:uniform} has to hold, an optimal social welfare is reached with $\hat{\sigma}$, which is still an NFCE since the constraints for Player 1 hold with equality.
%
Any other NFCE that may be reached when $a_1^T$ is played would lead to a social welfare of at most $c^*$. Indeed, the only difference from $\hat{\sigma}$ may be playing multiple truth assignments with strictly positive probability, whose linear combinations would result in $c^*$. Moreover, any probability distribution in which Player 1 does not play $a_1^T$ at $h_1^0$ provides social welfare 0 due to the payoff structure of $\Gamma_{\overline{c}}$.
	
($\overline{c}>c^*$). In this setting, $\Gamma_{\overline{c}}$ admits only NFCEs with social welfare 0. We observe that $\hat{\sigma}$ is no longer an NFCE of $\Gamma_{\overline{c}}$. Even if Property~\ref{prop:uniform} is still enforced, Player 1 is better off when selecting an action of type $a_1^{c_i}$ at $h_1^0$ (leading to a payoff of $\overline{c}$ against $c^*$, obtainable when playing $a_1^T$). The same holds for the other probability distributions in which $a_1^T$ is recommended to Player 1. Moreover, there always exists at least one NFCE with social welfare 0: it is enough to consider the normal-form game (derived from a portion of $\Gamma_{\overline{c}}$) with actions $\{a_1^{c_1},\ldots,a_1^{c_\eta}\}\times(\times_{j\in\{1,\ldots,m\}} \rho(h_1^{v_j}))$ for Player 1 and $P_2$ for Player 2. In this game, a probability distribution where the clauses at $h_2^0$ and $h_1^0$ are recommended uniformly to each players is an NE, and therefore an NFCE of $\Gamma_{\overline{c}}$.


Now, we employ $\Gamma$ to derive the inapproximability result. Assume, by contradiction, that there exists a polynomial-time approximation algorithm $\mathcal{A}$ providing an approximate solution to \textsf{NFCE-SW} with approximation factor $r=\frac{1}{f(\eta)}$, and let $f(\eta)=2^\eta$ (notice that the polynomiality of the process is preserved as $f(\eta)$ can be codified with $\eta$ bits). Let us proceed iteratively by setting $\overline{c}=1$, and increasing its value by 1 at each step, until we reach $\overline{c}=\eta$. For each value of $\overline{c}$, we run $\mathcal{A}$ over $\Gamma_{\overline{c}}$. If $\overline{c}<c^*$ (case 1), we obtain a solution which is greater than or equal to $\frac{c^*}{f(\eta)}$ and, therefore, it is strictly greater than 0. If $\overline{c}=c^*$ (case 2), $\mathcal{A}$ returns $\frac{c^*}{f(\eta)}$, which is, again, strictly greater than 0. If $\overline{c}>c^*$ (case 3), $\mathcal{A}$ returns 0. If we denote by $c^0$ the first value of $\overline{c}$ for which $\mathcal{A}$ returns 0, then we have (in polynomial time in the size of $\phi$) $c^*=c^0-1$. 
This leads to a contradiction as, if $\mathcal{A}$ existed, \textsf{MAX-SAT}--- which is known to be \textsf{NP}-hard --- would be solvable in polynomial time.
\end{proof}

